Numerical analysis of optimal control problems governed by fourth-order linear elliptic equations using the Hessian discretisation method

This paper focusses on the optimal control problems governed by fourth-order linear elliptic equations with clamped boundary conditions in the framework of the Hessian discretisation method (HDM). The HDM is an abstract framework that enables the convergence analysis of numerical methods through a quadruplet known as a Hessian discretisation (HD) and three core properties of HD. The HDM covers several numerical schemes such as the conforming finite element methods, the Adini and Morley non-conforming finite element methods (ncFEMs), method based on gradient recovery (GR) operators and the finite volume methods (FVMs). Basic error estimates and superconvergence results are established for the state, adjoint and control variables in the HDM framework. The article concludes with numerical results that illustrates the theoretical convergence rates for the GR method, Adini ncFEM and FVM.

==> Makefile <==
# Makefile pour compiler un .tex en .pdf
# 	MAIN = nom (sans extension .tex) du fichier principal
#	FIG = fichiers figures dont depend le $(MAIN)
# 	BIB = fichier .bib, s'il existe

MAIN = Fourth_order_elliptic_linear
FIG = $(wildcard *.pdf_t) $(wildcard pictures/*.png)
BIB = $(shell grep '\\bibliography{' $(MAIN).tex | sed s/'\\bibliography{'// | cut -d '}' -f 1 | sed s/"\.bib"/""/).bib

all: $(MAIN).pdf


# Cibles speciales: fichiers ne devant pas etre effaces, cibles
# non-fichiers et suppression de toutes les regles implicites
.PRECIOUS: %.aux %.bbl
.PHONY: clean voir edit
.SUFFIXES:

#
# Compiler le pdf
#
%.pdf: %.tex %.aux %.log $(FIG)
	-pdflatex -shell-escape $<

# .log marque comme prerequis mais sans regle pour etre reconnu
# comme fichier temporaire a supprimer une fois le pdf cree
%.log: ;

## En cas d'index (rajouter %.ind comme dependence au %.pdf)
##
#%.ind: %.tex
#	makeindex $(MAIN).idx

# Selon qu'il existe un fichier biblio ou pas, le .aux en depend ou pas
ifneq ($(strip $(wildcard $(BIB))),)
%.aux: %.tex %.bbl
	-pdflatex $<
else
%.aux: %.tex
	-pdflatex $<
endif

%.bbl: %.tex $(BIB)
	-pdflatex $<
	-bibtex $*

#
# Afficher le pdf
#		On copie d'abord dans un autre pdf, "view", pour eviter que des reload empechent
#		de voir pendant la compilation de latex
#
view-$(MAIN).pdf: $(MAIN).pdf
	cp $(MAIN).pdf view-$(MAIN).pdf;

voir: view-$(MAIN).pdf
	evince view-$(MAIN).pdf &

#
# Editer le tex
#
edit:
	gedit --new-window $(MAIN).tex &

#
# Voir le pdf et editer le tex
#
init: 
	make -s edit;
	make -s voir;

#
# Nettoyage
#
clean:
	rm -f $(MAIN).aux $(MAIN).log $(MAIN).bbl $(MAIN).blg $(MAIN).pdf view-$(MAIN).pdf




